Elucidating the Role of Filament Turnover in Cortical Flow using Simulations and Representation Learning

Cell polarization relies on long-range cortical flows, which are driven by active stresses and resisted by the cytoskeletal network. While the general mechanisms that contribute to cortical flows are known, a quantitative understanding of the factors that tune flow speeds has remained lacking. Here, we combine physical simulation, representation learning, and theory to elucidate the role of actin turnover in cortical flows. We show how turnover tunes the actin density and filament curvature and use representation learning to demonstrate that these quantities are sufficient to predict cortical flow speeds. We extend a recent theory for contractility to account for filament curvature in addition to the nonuniform distribution of crosslinkers along actin filaments due to turnover. We obtain formulas that can be used to fit data from simulations and microscopy experiments. Our work provides insights into the mechanisms of contractility that contribute to cortical flows and how they can be controlled quantitatively.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> recycle.tex <==
% Tension is generated within the cortex by assemblies of non-muscle myosin II pulling on actin filaments. 
% Cell shape and cell-cell interactions both depend on the  cortical tension, and tension gradients can give rise to long-range flows that transport proteins for cell polarization \cite{munro2004cortical,lang2017proteins}, migration \cite{hernandez2017polarized}, and division.   
%Understanding the underlying physical forces and stresses during this fundamental biological processes will foster advances in the development of optimal dynamic control of self-organized actomyosin contractility in cell polarization.  


% The emergence of long-range cortical flow can be attributed to the buildup of localized active stress with a polarization gradient, which works against internal viscous resistance~\cite{juelicher2007active,joanny2009active, banerjee2017actomyosin, malik2019scaling}.
% However, it is not fully understand how the balance between active force and internal resistance in actin cortex is regulated by the microscopic interactions of myosin, actin and crosslinkers. 
%This balance of active force and internal resistance leads to local deformations. Spatiotemporal control of cortical deformations drives changes in cell shape, cell movements, and intracellular transport

%Both directed and chaotic long-range flows have been reported for \textit{in vivo} ~\cite{munro2004cortical, maroudas2021topological} and \textit{in vitro}  ~\cite{malik2019scaling, zhang2021spatiotemporal,opathalage2019self} actomyosin networks. 
%The origin of chaotic flow is well studied, where local contractility is caused by the sliding of myosin on short actin filaments~\cite{Stam_Freedman_Banerjee_Weirich_Dinner_Gardel_2017}.
%The short actin filaments are aligned due to myosin activity and form active liquid crystal. The resulting chaotic flow is driven by the topological defects in the active nematics~\cite{zhang2021spatiotemporal} and has been shown to coincide with the emergence of morphological features in Hydra morphogenesis~\cite{maroudas2021topological}.

%In contrast, the microscopic origin of directed cortical flows in disordered actomyosin network is still an open challenge.   
%Different from the flow in active nematics,  maintaining the directed flow not only depends on myosin motors, but it also requires the activity of actin turnover~\cite{mcfadden2017filament}. 
%The directed cortical flow transports partitioning defective proteins to establish the cellular polarity~\cite{munro2004cortical} and is driven by the self-stabilizing polarized distribution of myosin proteins along the anterior-posterior axis~\cite{lang2017proteins}.  
%Actin turnover works as another resource of activity and releases the local active stress in the highly connected network~\cite{mcfadden2017filament} to avoid the network collapse~\cite{belmonte2017theory,malik2019scaling}.

%The local stress in this highly connected cortical network is generated via motor stress-induced filament buckling. Polarized distribution of myosins leads to a gradient of filament buckling, which in turn couples with the actin turnover dynamics and modulates the magnitude of the flow. 
%Existing theoretical frameworks  make predictions of the long-range flow by accounting for the active stress and viscosity of actin networks. However, it is non-trivial to determine the specific experimental conditions in which the theory framework is valid and can be applied to elucidate the underlying physics. 
%these predictions do not align with the observed flow in the simulations. This is partially because simulation imaging data are noisy and extracting the salient features behind the flow physics is challenging. 
%Representation learning allows us to overcome the obstacle. We find a latent representation of flow imaging and use it to refine the theoretical framework that provides a microscopic insight of the contractility mechanism and the control knobs of the flow intensity. 

% The same flow has been observed in in vitro actomyosin netroks as well~\cite{malik2019scaling}. However, The local contraction induced by actin buckling is not balanced by the actin turnover, resulting in the global contraction 
%Macroscopic from the posteriory pole to the anterior pole of the embryo, happens over minutes. 
%Higher RhoA at the anterior regions and  this flow during maintenance phase is driven by myosin gradient
%Our simulations indicate that filament turnover mainly modulates actin density and actin buckling. 
% In what follows, we use a machine learning technique to analyze simulations imaging, to understand how actin properties vary the active stress $\sigma_{a}$  and fluid viscosity $\eta$ in ~\cref{eq:sigma_eta_ratio}. 
% These simulations provide a platform beyond experiments to pursue how the perturbation of the cortex dynamics affect cortical flow. The analysis suggests that the effect of filament turnover on the rate of cortical flow is mediated by the modulation of actin density and buckling. 
% The features behind the contractility extracted by CNN autoencoder and UMAP are consistent with those suggested by the minimal theoretical model in the next section. Hence, we use these features to identify the physics and validate a theoretical model which further elucidates the roles of actin turnover and myosin gradient in controlling the cortical flows.
% Using these features extracted by CNN autoencoder and UMAP, we refine a theoretical framework in the next section to further elucidate the roles of actin turnover and myosin gradient in controlling the cortical flows.
% Combining these features extracted by CNN autoencoder and UMAP with the theoretical model in \cref{eq:sigma_eta_ratio}, we provide a refined model that elucidates of the effect of filament of actin turnover of cortical flows in the next section. \par
%that can support  physical theory, and may assist us to refine and improve an existing theoretical model.
% It has been proposed that distinct timescales of actin turnover and myosin activity affect active force transmission and deformation resistance in the actin cortex~\cite{mcfadden2017filament}. This suggests that the dependence of The cortical flow on the actin turnover is a combined effect of forces generated by active and resistant stresses.
%This equation indicates that the coupling between actin turnover and the myosin gradient causes the active stress and fluid viscosity to vary differently, resulting in a nonmonotonic shift in their ratio.
% In this study, the physical meaning of $\rho_{0}$ is the threshold under which the actin network experiences local tearing.  $f_{X}^0$ and $f_{X}^1$ denote the friction forces exerted by crosslinkers on each actin binding position with a uniform crosslinker distribution and accumulated crosslinkers at the filament ends, respectively. Due to excess amount of crosslinkers in the cortex, these two terms are considered independent of actin densities. 
% We assume uniformly 



% The force exerted by the motors depends on the number of motors per actin filament:  
% \begin{equation}
% f_M = \gamma_{M} \bar C_M /(\rho_a-\rho_0),
% \end{equation}
% where $\gamma_M$ is the exerted friction force per myosin.  

% Actin turnover modulates the overall actin densities, so we use a scaling constant $\lambda$  to replace the density term  $\rho_a - \rho_0$ with actin turnover rate $\lambda (k_a - k_0)$. $k_0$ is an actin turnover threshold below which actin filaments disassemble before myosin-induced forces can propagate. 
% However, applying this model to the simulations does not directly result in an interpretable model that captures the magnitude of the contractility (\textbf{SI}). We need to incorporate the insight from the latent representation into the theoretical framework.  
% The feature space identifies that actin turnover rate that gives rise to the maximized flow rate also provides the highest degree actin buckling in the network. This is consistent with the theory where the flow rate $d$ is proportional to the active stress (\cref{eq:sigma_eta_ratio}). 
%Simulations have been deployed to understand how actin turnover dynamics and motor activities cooperatively control the contractility of actin networks by regulating the active stress and viscous resistance~\cite{mcfadden2017filament}. These 
%This tension holds the cell cortex far from equilibrium and drives the cortex deformation.
%All these efforts aim to bring together theory and experiments/simulations to decode physics.
%Nevertheless, due to limited access to the microscopic measurement of active mechanics in the actin cortex in experiments, the mechanism of contractility and force generation that regulate the directed long-range cortical flow is not fully understood.  
